Pixel-Face: A Large-Scale, High-Resolution Benchmark for 3D Face Reconstruction

3D face reconstruction is a fundamental task that can facilitate numerous applications such as robust facial analysis and augmented reality. It is also a challenging task due to the lack of high-quality datasets that can fuel current deep learning-based methods. However, existing datasets are limited in quantity, realisticity and diversity. To circumvent these hurdles, we introduce Pixel-Face, a large-scale, high-resolution and diverse 3D face dataset with massive annotations. Specifically, Pixel-Face contains 855 subjects aging from 18 to 80. Each subject has more than 20 samples with various expressions. Each sample is composed of high-resolution multi-view RGB images and 3D meshes with various expressions. Moreover, we collect precise landmarks annotation and 3D registration result for each data. To demonstrate the advantages of Pixel-Face, we re-parameterize the 3D Morphable Model (3DMM) into Pixel-3DM using the collected data. We show that the obtained Pixel-3DM is better in modeling a wide range of face shapes and expressions. We also carefully benchmark existing 3D face reconstruction methods on our dataset. Moreover, Pixel-Face serves as an effective training source. We observe that the performance of current face reconstruction models significantly improves both on existing benchmarks and Pixel-Face after being fine-tuned using our newly collected data. Extensive experiments demonstrate the effectiveness of Pixel-3DM and the usefulness of Pixel-Face.

==> equation/ARMSE.tex <==
\begin{equation} \label{eq:ARMSE}
\begin{aligned}
& E(X_i, Y) = \min({\left\| X_i - Y_v\right\|}_2, {\left\| X_i - Y_e\right\|}_2, {\left\| X_i - Y_f\right\|}_2) \\
& \operatorname{ARMSE}(X, Y) =\left( \sqrt{\frac{\sum_{i=0}^{N_X} E\left(X_{i},Y\right)^{2}}{{N_{x}}}}+\sqrt{\frac{\sum_{i}^{N_{y}} E\left(Y_{j}, X\right)^{2}}{N_{y}}}\right) / {2 d}.
\end{aligned}
\end{equation}

==> paper_figures/pixel_face.tex <==
% !TEX root = ../main.tex


\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=0.95\linewidth]{figures/pixel_face.pdf}
	\end{center}
%	\vspace{-16pt}
	\caption{We qualitatively compare {\methodname}  with BFM17~\cite{gerig2018morphable} and FWH~\cite{cao2013facewarehouse} on the evaluation set of {\datasetname}, showing 3DMM fitting results and error maps. The results show that {\methodname} can better handle novel face shape and exaggerate expressions than previous counterparts.}
	\label{fig:pixel_face}
\end{figure*}


==> paper_figures/reg_overview.tex <==
% !TEX root = ../main.tex


\begin{figure*}[tb]
	\centering
	\includegraphics[width=1\linewidth]{figures/reg_overview.pdf}
	\vspace{-16pt}
	\caption{Comparison of spatial-varying and normal NICP registration results. The left is the face parsing region map and corresponding stiffness weight. The normal NICP breaks the coherence of topology so we can see the artificial wrinkle in surface. The comparison illustrate the spatial-varying algorithm yields more smooth and fitting registration.}
	\label{fig:reg_overview}
\end{figure*}


==> tables/age_expression.tex <==
% !TEX root = ../main.tex


\begin{table}[t] \centering \small
	\caption{NME and ARMSE scores with state-of-the-art face 3D reconstruction methods, under different age region and different crop radius.}
    \setlength\tabcolsep{3pt}
	\begin{tabular}{ccccccc}
		\toprule
		\multicolumn{2}{c}{Evaluation $\rightarrow$} & \multicolumn{5}{c }{ARMSE$\&$NME}  \\ \cline{3-7} 
		\multicolumn{2}{c}{Methods $\downarrow$} & \multicolumn{1}{c}{1-20} & \multicolumn{1}{c}{21-40} & \multicolumn{1}{c}{41-60} & \multicolumn{1}{c}{$>$60} & \multicolumn{1}{c}{Ave} \\ \hline
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.6}} & 3DDFA~\cite{zhu2017face} & $3.29/4.68$ & $3.45/4.43$ & $3.67/4.64$ & $3.71/4.72$ & $3.57/4.57$ \\
		\multicolumn{1}{l}{} & PRNet~\cite{feng2018prn} & $3.56/4.61$ & $3.50 / 4.37$ & $3.65 /4.46$ & $3.59 /4.52$ & $3.56 /4.44$ \\ 
		\multicolumn{1}{l}{} & RingNet\cite{RingNet:CVPR:2019} & $4.35/5.85$ & $4.67/5.59$ & $4.87/5.70$ & $4.82/5.67$ & $4.74/5.65$\\ 
		\hline
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.7}} & 3DDFA & $3.59/4.69$ & $3.73/4.43$ & $4.03/4.64$ & $4.13/4.72$ & $3.90/4.57$  \\
		\multicolumn{1}{l}{} & PRNet & $3.52 / 4.62$ & $3.66 / 4.38$ & $3.84 / 4.45$ & $3.84 / 4.52$ & $3.75/4.44$ \\ 
		\multicolumn{1}{l}{} & RingNet & $5.18/5.86$ & $5.27/5.59$ & $5.54/5.68$ & $5.54/5.67$ & $5.40/5.65$ \\
		\hline
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.8}} & 3DDFA & $3.95/4.69$ & $4.06/4.43$ & $4.49/4.64$ & $4.62/4.72$ & $4.31/4.56$ \\
		\multicolumn{1}{l}{} & PRNet & $3.88 / 4.61$ & $3.94 / 4.37$ & $4.17 / 4.45$ & $4.20 / 4.51$ & $4.06/4.44$  \\ 
		\multicolumn{1}{l}{} & RingNet & $6.46/5.87$ & $6.24/5.59$ & $6.60/5.63$ & $6.66/5.63$ & $6.45/5.62$\\
		\hline	
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.9}} & 3DDFA & $4.37/4.67$ & $4.39/4.43$ & $4.92/4.62$ & $5.11/4.71$ & $4.70/4.55$ \\
		\multicolumn{1}{l}{} & PRNet & $4.39 / 4.60$ & $4.35 / 4.36$ & $4.61 /4.44$ & $4.73 / 4.51$ & $4.51 / 4.43$\\ 
		\multicolumn{1}{l}{} & RingNet & $7.55/5.78$ & $7.34/5.54$ & $7.65/5.60$ & $7.75/5.58$ & $7.52/5.58$  \\
		\hline	
		\multicolumn{1}{l}{\multirow{3}{*}{r=1.0}} & 3DDFA & $4.81/4.66$ & $4.67/4.42$ & $5.19/4.59$ & $5.44/4.69$ & $4.99/4.54$  \\
		\multicolumn{1}{l}{} & PRNet & $4.82 / 4.58$ & $4.69 / 4.35$ & $5.00 / 4.42$ & $5.16 / 4.50$ & $4.89 / 4.41$  \\ 
		\multicolumn{1}{l}{} & RingNet & $7.66/5.78$ & $7.34/5.50$ & $7.64/5.59$ & $7.78/5.51$ & $7.52/5.54$  \\
		\bottomrule
	\end{tabular}
	\label{tab:age_region}
\end{table}


\begin{table}[t] \centering
	\caption{NME and ARMSE scores with state-of-the-art face 3D reconstruction methods, under different expression region and different crop radius.}
	\setlength\tabcolsep{3pt}
	\begin{tabular}{cccccc}
		\toprule
		\multicolumn{2}{c}{Evaluation $\rightarrow$} & \multicolumn{4}{c }{ARMSE$\&$NME}  \\ \cline{3-6} 
		\multicolumn{2}{c}{Methods $\downarrow$} & \multicolumn{1}{c}{Neutral} & \multicolumn{1}{c}{Positive} & \multicolumn{1}{c}{Negative} &  \multicolumn{1}{c}{Ave} \\ \hline
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.6}} & 3DDFA~\cite{zhu2017face} & $3.51/4.64$ & $3.63/4.53$ & $3.57/4.55$ & $3.57/4.57$  \\
		\multicolumn{1}{l}{} & PRNet~\cite{feng2018prn} & $3.35/4.25$ & $3.45/4.48$ & $3.66/4.49$ & $3.56/4.44$ \\ 
		\multicolumn{1}{l}{} & RingNet\cite{RingNet:CVPR:2019} & $4.71/5.48$ & $4.71/5.72$ & $4.78/5.68$ & $4.75/5.65$ \\ 
		\hline
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.7}} & 3DDFA & $3.87/4.64$ & $3.63/4.53$ & $3.57/4.45$  & $3.57/4.55$  \\
		\multicolumn{1}{l}{} & PRNet & $3.49/4.25$ & $3.72/4.48$ & $3.84/4.49$ & $3.75 / 4.44$  \\ 
		\multicolumn{1}{l}{} & RingNet & $5.29/5.48$ & $5.51/5.71$ & $5.41/5.68$ & $5.40/5.65$ \\
		\hline
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.8}} & 3DDFA & $4.31/4.64$ & $4.31/4.53$ & $4.31/4.55$ & $4.31/4.56$  \\
		\multicolumn{1}{l}{} & PRNet & $3.78/4.25$ & $4.12/4.48$ & $4.13/4.49$ & $4.06/4.44$  \\ 
		\multicolumn{1}{l}{} & RingNet & $6.30/5.47$ & $6.58/5.66$ & $6.46/5.66$ & $6.46/5.62$ \\
		\hline	
		\multicolumn{1}{l}{\multirow{3}{*}{r=0.9}} & 3DDFA & $4.75/4.62$ & $4.69/4.52$ & $4.69/4.54$ & $4.70/4.55$  \\
		\multicolumn{1}{l}{} & PRNet & $4.21/4.24$ & $4.66/4.47$ & $4.57/4.47$ & $4.51/4.43$\\ 
		\multicolumn{1}{l}{} & RingNet & $7.46/5.46$ & $7.54/5.57$ & $7.53/5.62$ & $7.52/5.58$ \\
		\hline	
		\multicolumn{1}{l}{\multirow{3}{*}{r=1.0}} & 3DDFA & $5.07/4.60$ & $4.96/4.51$ & $4.97/4.53$ & $4.99/4.54$   \\
		\multicolumn{1}{l}{} & PRNet & $4.58/4.24$ & $5.02/4.44$ & $4.95/4.46$ & $4.89/4.41$  \\ 
		\multicolumn{1}{l}{} & RingNet & $7.47/5.46$ & $7.57/5.52$ & $7.54/5.58$ & $7.52/5.54$   \\
		\bottomrule
	\end{tabular}
	\label{tab:exp_region}
\end{table}

==> tables/facenet.tex <==
% !TEX root = ../main.tex

\begin{table}[ht] \centering  %\small % 
	\caption{We quantitatively compare 2D face recogition performance of PRNet~\cite{feng2018prn} with and without finetuned on our data and LFW~\cite{Huang2012a}. The results show that fine-tuning on {\datasetname} increase the identity consistent ability.
	}
 
	\vskip 0.2 cm
	\setlength\tabcolsep{5pt}
	\begin{tabular}{ccc}
		\toprule
	      &   \datasetname & LFW\\
		\hline
		 w/o finetune	&	$0.69$ &	$0.81$ \\
		 with finetune & \textbf{$0.76$} & \textbf{$0.84$} \\
		\bottomrule
	\end{tabular}	
	\label{tab:facenet}
%	\vspace{0 cm}
\end{table}


